Truth Inference on Sparse Crowdsourcing Data with Local Differential Privacy

Crowdsourcing has arisen as a new problem-solving paradigm for tasks that are difficult for computers but easy for humans. However, since the answers collected from the recruited participants (workers) may contain sensitive information, crowdsourcing raises serious privacy concerns. In this paper, we investigate the problem of protecting answer privacy under local differential privacy (LDP), by which individual workers randomize their answers independently and send the perturbed answers to the task requester. The utility goal is to enable to infer the true answer (i.e., truth) from the perturbed data with high accuracy. One of the challenges of LDP perturbation is the sparsity of worker answers (i.e., each worker only answers a small number of tasks). Simple extension of the existing approaches (e.g., Laplace perturbation and randomized response) may incur large error of truth inference on sparse data. Thus we design an efficient new matrix factorization (MF) algorithm under LDP. We prove that our MF algorithm can provide both LDP guarantee and small error of truth inference, regardless of the sparsity of worker answers. We perform extensive experiments on real-world and synthetic datasets, and demonstrate that the MF algorithm performs better than the existing LDP algorithms on sparse crowdsourcing data.

==> rrlaplace.tex <==
\subsection{Combined Approach (RR+LP)}
\label{sc:rrlp}
% general idea and advantage
Both LP and RR approaches have their drawbacks. The main weakness of the LP approach is its treatment of NULL values. By replacing the large fraction of NULL values, the LP approach may change the answer distribution significantly and incur large inaccuracy on the inferred truths. On the other hand, 
the main weakness of the RR mechanism is its handling of non-NULL values. Since it replaces the non-NULL answers with random values in the domain, it may lead to large errors in truth inference result when the truth is not around the center of the domain. 
To address these limitations, we design the third straw-man approach named RR+LP, which integrates LP and RR. The RR+LP method is a two-step process. First, the algorithm decides if the original worker answer is perturbed to one of the two {\em classes}, namely non-NULL and NULL, by using the RR approach. 
If Step 1 chooses the answer class as non-NULL, in Step 2, the LP approach is applied on the original answer for perturbation.  
	% keep NULL, avoid bias
Intuitively, this design can help eliminate the shortcomings of both LP and RR approaches. First, compared with the LP approach, RR+LP preserves NULL values to some extent, and thus reduces the amounts of perturbation on the worker answers. Second, unlike RR, it does not replace non-NULL answers with a random guess in the domain. Thus it reduces the perturbation on the distribution of original non-NULL answers. Next, we present the details of the two-step RR+LP approach.
   
% detail
% step 1
\noindent{\bf Step 1. Class perturbation by RR.} For a given answer $a_{ij}$ that belongs to either the NULL or non-NULL class, Step 1 decides which class (NULL or non-NULL) the perturbed value of $a_{ij}$ belongs to by the following design matrix:
\begin{equation}
P^A = 
\kbordermatrix{
    Input\backslash Output & NULL & NON-NULL \\
    NULL & \frac{e^{\epsilon_1}}{1+e^{\epsilon_1}} & \frac{1}{1+e^{\epsilon_1}} \\
    NON-NULL & \frac{1}{1+e^{\epsilon_1}} & \frac{e^{\epsilon_1}}{1+e^{\epsilon_1}}
    },
\end{equation}
where $\epsilon_1>0$ is the privacy budget for the class perturbation. 
%Following this design, the NULL values are more likely to be kept NULL in the perturbed answer vector. 

\noindent{\bf Step 2. Adding Laplace noise.} If the output of Step 1 is the non-NULL class, the perturbed $a_{i,j}$ is generated by adding Laplace noise with the privacy parameter $\epsilon_2$. If $a_{i,j}$ is NULL, a random value is uniformly randomly picked from the domain $\Gamma$ prior to perturbation.
%answer is $g(a_{ij})+Lap(\frac{|\Gamma|}{\epsilon_2})$, where $g(\dot)$ is per Equation (\ref{eq:g}), and $\epsilon_2>0$ is the privacy budget to produce a NON-NULL answer.

The following theorem shows that the RR+LP mechanism satisfies $(\epsilon_1+\epsilon_2)$-LDP.

\begin{theorem}
\label{thm:rrlp_dp}
The RR+LP mechanism guarantees $(\epsilon_1+\epsilon_2)$-LDP.

\begin{proof}
%Similar to the proof of Theorem \ref{thm:rr_dp}, we prove that for any pair of answer vectors $\vec{a}_i$ and $\vec{a}_j$ that differ at the first element, $\frac{Pr[\mathcal{M}(\vec{a}_i)=\vec{z}_p]}{Pr[\mathcal{M}(\vec{a}_j)=\vec{z}_p]}\leq e^{\epsilon_1+\epsilon_2}$. 
According to the two-step perturbation mechanism, we have 
\begin{equation*}
\begin{aligned}
& Pr[\mathcal{M}(a_{i,j})=y] \\ 
= &
	\begin{cases}
	\frac{1}{1+\exp(\epsilon_1)} & \text{ if } a_{i,j}\neq NULL\text{ and } y=NULL \\
    \frac{\exp(\epsilon_1)}{1+\exp(\epsilon_1)} & \text{ if } a_{i,j}=NULL\text{ and } y=NULL \\
    \frac{\exp(\epsilon_1)\exp(-\mid y-a_{i,j}\mid \frac{\epsilon_2}{|\Gamma|})}{1+\exp(\epsilon_1)} & \text{ if } a_{i,j}\neq NULL \text{ and } y\neq NULL \\
    \frac{\exp(-\mid y-x\mid \frac{\epsilon_2}{|\Gamma|})}{1+\exp(\epsilon_1)} & \text{ if } a_{i,j}=NULL \text{ and } y\neq NULL 
	\end{cases}
\end{aligned}
\end{equation*}
where $x\sim \mathcal{U}(\Gamma)$ is a value uniformly sampled from $\Gamma$.

Since 
\[\frac{\exp(\epsilon_1-\epsilon_2)}{1+\exp(\epsilon_1)}\leq \frac{\exp(\epsilon_1)\exp(-\mid y-a_{i,j}\mid \frac{\epsilon_2}{|\Gamma|})}{1+\exp(\epsilon_1)} \leq \frac{\exp(\epsilon_1)}{1+\exp(\epsilon_1)}, \]
and
\[\frac{\exp(-\epsilon_2)}{1+\exp(\epsilon_1)} \leq \frac{\exp(-\mid y-x\mid \frac{\epsilon_2}{|\Gamma|})}{1+\exp(\epsilon_1)}\leq \frac{1}{1+\exp(\epsilon_1)},\]
we can infer that 
\begin{equation*}
\frac{Pr[\mathcal{M}(a_{i,j})=y]}{Pr[\mathcal{M}(a_{i,j}')=y]} \leq
\begin{cases}
\exp(\epsilon_1) & \text{ if } y=NULL \\
\exp(\epsilon_1+\epsilon_2) &  \text{ if } y\neq NULL
\end{cases}
\end{equation*}
Therefore, RR+LP guarantees $(\epsilon_1+\epsilon_2)$-LDP.
\end{proof}
\end{theorem}    

Next, we show the expected error bound of the RR+LP approach. 
\begin{theorem}
\label{thm:rrlp_bound}
The expected error $E\left[MAE(\{\hat{a}_j\})\right]$ of estimated truth based on the answer vectors perturbed by the RR+LP mechanism satisfies:
\[E\left[MAE(\{\hat{a}_j\})\right] \leq \frac{1}{n}\sum_{j=1}^{n}\frac{\sum_{W_i\in \overline{W_{j}}}q_i\times e_{i,j}^{RR+LP}}{\sum_{W_i\in \overline{W_{j}}}q_i},\] 
where 
\begin{equation*}
\begin{aligned}
&e_{i,j}^{RR+LP}=\\
&\frac{1}{s_i+e^{\epsilon_1}(1-s_i)}\left(s_i\psi_{\mu_j}(\Gamma)+s_i\frac{|\Gamma|}{\epsilon_2}+e^{\epsilon_1}(1-s_i)\left(\sigma_i\sqrt{\frac{2}{\pi}}+\frac{|\Gamma|}{\epsilon_2}\right)\right),
\end{aligned}
\end{equation*}
$s_i$ is the fraction of tasks that worker $W_i$ returns non-NULL values, $\psi_{\mu_j}(\Gamma)=\frac{(max-\mu_j)^2+(\mu_j-min)^2}{2(max-min)}$, and $min$ and $max$ are the minimum and maximum value of $\Gamma$.
\end{theorem}
The proof of Theorem \ref{thm:rrlp_bound} is included in our full paper \cite{sun2018truth}. 
\nop{
\Wendy{1. The theorem is super complicated. How large the error bound can be for some specific settings? 2. I checked the proof. I don't understand how Step 1 goes to Step 2.}

\Boxiang{The bound is pretty loose. It is similar to LP, but much larger than RR. We checked the proof. There are two relaxations, while in RR, there is only one relaxation. So even though in practice, RR+LP is better than RR when $u_j=4.5$, the theoretical bounds are the opposite.}
\begin{tabular}{|c|c|c|}
\hline
$\epsilon=1$ & $\mu_j=4.5$ & $\mu_j=0$ \\\hline 
$s_i=0.1$ & 12.04 & 12.24 \\\hline
$s_i=0.9$ & 13.19 & 15.2 \\\hline
\end{tabular}
\begin{tabular}{|c|c|c|}
\hline
$\epsilon=5$ & $\mu_j=4.5$ & $\mu_j=0$ \\\hline 
$s_i=0.1$ & 3.14 & 3.28 \\\hline
$s_i=0.9$ & 4.275 & 6.176 \\\hline
\end{tabular}
}

\nop{
The two straw-man approaches both have their disadvantages. On one hand, for LP, it can only deal with numeric values and therefore cannot give any privacy protection between NULL values and normal values without filling a default value on the NULL cells. However, filling default values will reduce the final utility of the truth inference algorithm. On the other hand, for RR, which can give privacy protect for both NULL values and normal values. Regrettably, RR can only deal with discrete domain of answer. Further more, when applying privacy protection between normal values, this approach will assign highest picking probability to the original value, and assign uniform probabilities to all other possible values. Unlike the Laplace noise, this procedure is unfair to those possible values that are closer to the original one, which could also downgrade the utility.

Following the idea that highlighting the advantages and avoiding the disadvantages, we combine them together to be a new approach, RR+LP. The basic idea is, we pick the first step of RR, which preserves the privacy between NULL values and normal values with privacy budget $\epsilon_1$. After this step, we assign a Laplace noise with privacy budget $\epsilon_2$, $Lap\left(\frac{\Delta}{\epsilon_2}\right)$, to all the remaining normal values, even they might not be normal values originally. Since we apply two step differential privacy with budget $\epsilon_1$ and $\epsilon_2$, obviously each cell will satisfy at least $\epsilon_1$-DP and therefore we can say each cell have ($\epsilon_1+\epsilon_2$)-DP.

As we mentioned above, this approach avoid the disadvantages of LP and RR. LP+RR can handle both discrete and continuous domain. The cells with originally NULL value can have higher probability to retain their values, rather than randomly pick one to hurt the final utility. However, the disadvantage is, the protection between normal values in the second step uses privacy budget $\epsilon_2$, which is smaller than the total. Therefore when we want to apply the same totally budget to a dataset and the total budget $\epsilon$ is very small, the performance of RR+LP might not as good as LP or RR.
}
